$i$REPO: $i$mplicit Reward Pairwise Difference based Empirical Preference Optimization

While astonishingly capable, large Language Models (LLM) can sometimes produce outputs that deviate from human expectations. Such deviations necessitate an alignment phase to prevent disseminating untruthful, toxic, or biased information. Traditional alignment methods based on reinforcement learning often struggle with the identified instability, whereas preference optimization methods are limited by their overfitting to pre-collected hard-label datasets. In this paper, we propose a novel LLM alignment framework named $i$REPO, which utilizes implicit Reward pairwise difference regression for Empirical Preference Optimization. Particularly, $i$REPO employs self-generated datasets labeled by empirical human (or AI annotator) preference to iteratively refine the aligned policy through a novel regression-based loss function. Furthermore, we introduce an innovative algorithm backed by theoretical guarantees for achieving optimal results under ideal assumptions and providing a practical performance-gap result without such assumptions. Experimental results with Phi-2 and Mistral-7B demonstrate that $i$REPO effectively achieves self-alignment using soft-label, self-generated responses and the logit of empirical AI annotators. Furthermore, our approach surpasses preference optimization baselines in evaluations using the Language Model Evaluation Harness and Multi-turn benchmarks.

==> math_content.tex <==
\section{Math Content}
To simplify notation, denote $\gF \defeq \ell \,\circ \, \gH \defeq \set{ z \mapsto \ell(z,h), h \in \gH }.$ 

We have
\begin{align}
	{\mathscr{L}(\widehat{P}_{\lambda}, f_{\theta}) :=
	\mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\theta})}} \\
{\mathscr{L}({P}, f_{\theta}) \defeq \mathbf{E}_{Z \sim {P}} \bigS{\ell(Z,  h_{\theta})}}. \\
{\mathscr{L}({P}, f) \defeq \mathbf{E}_{Z \sim {P}} \bigS{\ell(Z,  h)}}.
\end{align}

\begin{align}
\mathscr{L}_{\rho}^{\gamma} (\widehat{P}_{\lambda},f) := & \mathbf{E}_{Z \sim \widehat{P}_{\lambda}}\Big{[}\phi_\gamma(Z, h)\Big{]} + \gamma \rho \\
\mathscr{L}_{\rho}^{\gamma} ({P},f) := & \mathbf{E}_{Z \sim {P}}\Big{[}\phi_\gamma(Z, h)\Big{]} + \gamma \rho. 
\end{align}

\textbf{Raginsky}: Suppose that $f$ is $L$-Lipschitz
\begin{align}
\mathscr{L}(Q, f) &\leq \mathscr{L}_{\rho}(P_{\lambda},f) \leq \mathscr{L}(Q,f) + 2L\rho, \;\forall Q \in \gB(P_{\lambda}, \rho) \\
\mathscr{L}(Q, f) &\leq \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) \leq \mathscr{L}(Q,f) + 2L\rho, \;\forall Q \in \gB(P_{\lambda}, \rho)
\end{align}


\textbf{Proposition 1}: Suppose that $f$ is $L$-Lipschitz
\begin{align}
\mathscr{L}(Q,f) &\leq   \mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f) \leq  \mathscr{L}(Q,f) + (2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \, {\rho}, \;\forall Q \in \gB(P_{\lambda}, \rho) \\
%\mathscr{L}(Q,f) &\leq   \mathscr{L}(P_{\lambda},\phi_{\gamma}) \leq  \mathscr{L}(Q,f) + (2L + \gamma\mathbf{I}) \, {\rho}, \;\forall Q \in \gB(P_{\lambda}, \rho)
\end{align}

\begin{proof}
	The first inequality:
	\begin{align}
	\mathscr{L}(Q,f) \leq  \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f)  \leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f) \\
%	\mathscr{L}(Q,f) \leq  \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) \leq  \mathscr{L}(P_{\lambda},\phi_{\gamma})
	\end{align}
	
	The last "$ \leq $":
	
	\begin{align*} 
%	\mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f)  & =  \mathscr{L}_{\rho}(P_{\lambda},f) + \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f)  - \mathscr{L}_{\rho}(P_{\lambda},f) \\
	\mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f)   & =   \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) + \mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f)  - \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) \\
	&\leq   \mathscr{L}(Q,f) + 2L\rho  + \mathbf{E}_{Z \sim P}[\phi_{\gamma}(Z, h)] + \rho\gamma - \min_{\gamma^{\prime} \geq 0} \Big\{ \rho \gamma^{\prime} + \mathbf{E}_{Z \sim P}[\phi_{\gamma'}(Z, h)] \Big\} \\
	& \leq   \mathscr{L}(Q,f) + 2L\rho + \max_{\gamma^{\prime} \geq 0}\bigg\{{\rho}(\gamma - \gamma^{\prime}) + \mathbf{E}_{Z \sim P}\Big[\phi_{\gamma}(Z, h) - \phi_{\gamma'}(Z, h)\Big]\bigg\} \\
	& =  \begin{aligned}[t] \mathscr{L}(Q,f) + 2L\rho + \max_{\gamma^{\prime} \geq 0}\Bigg\{\rho(\gamma - \gamma^{\prime}) + \mathbf{E}_{Z \sim P}\bigg[& \sup_{\zeta \in \mathcal{Z}} \Big\{ \ell(\zeta,h)  - \gamma d(\zeta,  Z) \Big\} \\ 
		& \quad - \sup_{\zeta \in \mathcal{Z}} \Big\{ \ell(\zeta,h) - \gamma^{\prime} d(\zeta,  Z)  \Big\} \bigg]\Bigg\} \end{aligned} \\
	& =  \mathscr{L}(Q,f) + 2L\rho + \max_{\gamma^{\prime} \geq 0}\Bigg\{\rho(\gamma - \gamma^{\prime}) + \mathbf{E}_{Z \sim P}\bigg[\sup_{\zeta \in \mathcal{Z}} \Big\{(\gamma^{\prime} - \gamma) d(\zeta,  Z)\Big\}\bigg]\Bigg\} \\
	& =  \mathscr{L}(Q,f) + 2L\rho + \underbrace{\max_{k \leq \gamma}\Bigg\{k\bigg(\rho - \mathbf{E}_{Z \sim P}\Big[\sup_{\zeta \in \mathcal{Z}} d(\zeta,  Z)\Big]\bigg)\Bigg\}}_{A} \\
	& \leq   \mathscr{L}(Q,f) + (2L + \gamma \, \mathbbm{1}_{\{\gamma \neq \gamma^{\prime}\}})\rho
	\end{align*}
	
	where $ k = \gamma - \gamma^{\prime} \Rightarrow \gamma^{\prime} = \gamma - k \geq 0 $
	because 
	\[
	A \leq \left\{\begin{array}{cc}{\gamma}{\rho} & \text { if } \rho \geq \mathbf{E}_{Z \sim P}\Big[\underset{\zeta \in \mathcal{Z}}{\sup}\big\{d(\zeta, Z)\big\}\Big]  \Rightarrow k=\gamma \\ 
	 \\ 0 & \text { if } \rho < ... \ k=0\end{array}\right.
	\]
	
\end{proof}

\begin{lemma} Suppose that $f'$ is $L_z$-Lipschitz
	 \[
	 	 \mathscr{L}(Q, f') - \inf_{f \in \mathcal{F}} \mathscr{L}(Q, f) \leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f') - \inf_{f \in \mathcal{F}} \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) + (2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho, \; \forall Q \in \gB(P_{\lambda}, \rho). 
	 \]
	
\end{lemma}

\begin{proof}
	From proposition 1 and when $f_Q = \argmin_{f \in \mathcal{F}} \mathscr{L}(Q, f)$ is $L$-Lipschitz, we have:
	\begin{align}
		\mathscr{L}(Q, f') &\leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f'),  \\ 
		\inf_{f \in \mathcal{F}} \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) \leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f_Q) &\leq \mathscr{L}(Q, f_{Q}) + (2 L+\gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho \\
		&= \inf_{f \in \mathcal{F}} \mathscr{L}(Q, f) + (2 L+\gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho. 
	\end{align}
	where  

\end{proof}

%\begin{theorem} If Assumption $\ell(Z,f)$ is $L_{\theta}$-Lipschitz continuous, then 
%	\[ 
%		\mathscr{L}(P_{\lambda}, \widehat{f}_{\theta^{\sigma}})- \inf_{f \in \mathcal{F}} \mathscr{L}(P_{\lambda}, f) \leq  \frac{\mathscr{C}(\gF)}{\sqrt{n}}+\epsilon + M \sqrt{\frac{2 \log (2 / \delta)}{n}} + (2L + \gamma) \hat{\rho}
%	\]
%	where:  
%	$\mathcal{F} = \bigC{f_{\theta}, \theta \in \Theta  \subset \mathbb{R}^d}$ and  $ \widehat{f}_{\theta^{\sigma}} \in \underset{\theta \in \Theta}{\operatorname{argmin}}\ \mathscr{L}(\widehat{P}_{\lambda}, f_{\theta}) + \sigma$, and 
%	$\mathscr{C}(\mathcal{F}):=\int_{0}^{\infty} \sqrt{\log \mathcal{N}\left(\mathcal{F},\|\cdot\|_{\infty}, \epsilon \right)} \mathrm{d} \epsilon$ and $\mathcal{N}\left(\mathcal{F},\|\cdot\|_{\infty}, \epsilon \right)$ denotes the covering number of $\mathcal{F}$ in the uniform metric $\ldots$.
%\end{theorem}

\begin{theorem} \label{Thrm:key} If Assumption $\ell(z,h_{\theta})$ is $L_{\theta}$-Lipschitz continuous, $\abs{\ell(z,h) } \leq M_{\ell}$ and considering the parametrized hypothesis class  $\mathcal{H} = \bigC{h_{\theta}, \theta \in \Theta  \subset \mathbb{R}^d}$, and $\forall Q \in \gB(P_{\lambda}, \rho)$, then 
	\[ 
	\mathscr{L}(Q, {f}_{\widehat{\theta}^{\varepsilon}})- \inf_{f \in \mathcal{F}} \mathscr{L}(Q, f) \leq  \sum_{i=1}^{m} \lambda_i \BiggS{\frac{48 \mathscr{C}(\Theta)}{\sqrt{n_i}} + 2 M_{\ell} \sqrt{\frac{2 \log (2  m / \delta)}{n_i}}} +\varepsilon + (2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho
	\]
	with probability at least $1 - \delta$. Here $\widehat{\theta}^{\varepsilon}$ is the solution returned by FedRob after $O(1/\varepsilon)$ iterations, i.e., 
	  \begin{align}
	%  \mathscr{L}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) &\defeq \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\widehat{\theta}^{\varepsilon}})}  \leq \underset{\theta \in \Theta} {\operatorname{inf}} \ \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\theta})}  + \varepsilon \\
	  \mathscr{L}_{\rho}^{\gamma} (\widehat{P}_{\lambda},f_{\widehat{\theta}^{\varepsilon}})  & \defeq \mathbf{E}_{Z \sim \widehat{P}_{\lambda}}\Big{[}\phi_\gamma(Z, h_{\widehat{\theta}^{\varepsilon}})\Big{]} + \gamma \rho \leq \underset{\theta \in \Theta} {\operatorname{inf}}  \BigS{\mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\phi(Z,  h_{\theta})}  + \gamma \rho } + \varepsilon
%	  {\widehat{\theta}^{\varepsilon}} \in \underset{\theta \in \Theta} {\operatorname{argmin}} \ \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\theta})}  + \varepsilon
	  \end{align}
	  and 
	$\mathscr{C}(\Theta):= L_{\theta} \int_{0}^{\infty} \sqrt{\log \mathcal{N}\left(\Theta,\|\cdot\|_{\Theta}, \epsilon \right)} \mathrm{d} \epsilon$ where $\mathcal{N}\left(\Theta,\|\cdot\|_{\Theta}, \epsilon \right)$ denotes the $\epsilon$-covering number of $\Theta$ w.r.t  a  metric $\|\cdot\|_{\Theta}$ as the norm on $\Theta$.
\end{theorem}

\textbf{Remarks:}
Choose $\varepsilon$ in the order of $1/\sqrt{n}$. 

\begin{proof}
	To simplify notation, we denote $ \Phi \defeq \phi_{\gamma} \circ \mathcal{H} = \set{z \mapsto \phi_{\gamma}(z, h), h \in \mathcal{H}}$ where $\mathcal{H} = \bigC{h_{\theta}, \theta \in \Theta  \subset \mathbb{R}^d}$, which represents the composition of $\phi_{\gamma}$ with each of the predictor function $h_{\theta}$ parametrized by $\theta$ belonging to a parameter class $\Theta$. 
	
	Defining $f_P \in \argmin_{f \in \mathcal{F}} \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f)$ and $ \widehat{\theta}^* \in \underset{\theta \in \Theta} {\operatorname{argmin}} \ \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\phi(Z,  h_{\theta})}$ such that $\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^*}) = \underset{\theta \in \Theta} {\operatorname{inf}}  \BigS{\mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\phi(Z,  h_{\theta})}  + \gamma \rho }$, we  decompose the excess risk as follows:
	
	\begin{align}
	&\mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) - \inf_{f \in \mathcal{F}}  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) \nonumber\\
	&= \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) -   \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f_P)\nonumber\\
	&=  \BigS{\mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}})} + \underbrace{\BigS{\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{*}})} }_{\leq \varepsilon} + \underbrace{\BigS{\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{*}}) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, f_P)}}_{\leq 0} \nonumber\\
	& \quad  + \BigS{\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, f_P) - \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f_P)} \nonumber\\
%	& \leq 2 \sup_{f \in \mathcal{F}} \; \big\lvert\mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, f) \big\rvert  + \varepsilon\\
	&\leq 2 \sup_{\phi_{\gamma} \in \Phi} \abs*{ \mathbf{E}_{Z \sim P_{\lambda}}[\phi_{\gamma}(Z, h_{\theta})] -   \mathbf{E}_{Z \sim \widehat{P}_{\lambda}}[\phi_{\gamma}(Z, h_{\theta})] } + \varepsilon \nonumber\\
	&\leq 2 \sup_{\phi_{\gamma} \in \Phi}  \sum_{i=1}^{m} \lambda_i \abs*{\mathbf{E}_{Z_i \sim P_i}[\phi_{\gamma}(Z_i, h_{\theta})] -   \mathbf{E}_{Z_i \sim \widehat{P}_{i}}[\phi_{\gamma}(Z_i, h_{\theta})]}  + \varepsilon \nonumber\\
	&\leq 2   \sum_{i=1}^{m} \lambda_i \sup_{\phi_{\gamma} \in \Phi} \abs*{\mathbf{E}_{Z_i \sim P_i}[\phi_{\gamma}(Z_i, h_{\theta})] -   \mathbf{E}_{Z_i \sim \widehat{P}_{i}}[\phi_{\gamma}(Z_i, h_{\theta})]}  + \varepsilon \nonumber\\
	%&\stackrel{\text {with prob. } \geq 1-\delta}{\leq}  
	& \leq  \sum_{i=1}^{m} \lambda_i  \biggS{4 \mathscr{R}_{i}(\Phi)+  2 M_{\ell} \sqrt{\frac{2 \log (2 m / \delta)}{n_i}}} + \varepsilon\, \text{  with probability at least }  1-\delta, \label{unionbound1}
	\end{align}
where the first inequality is due to optimization error and definition of $\widehat{\theta}^{*}$. The second inequality is due to the fact that $ \abs{\sum_{i=1}^m \lambda_i a_i } \leq \sum_{i=1}^m \lambda_i  \abs{a_i}, \forall a_i \in \mathbb{R}$ and $\lambda_i \geq 0$. The third inequality is because pushing the $\sup$ inside increases the value. For the last inequality, using  the facts that (i) $\abs{\phi_{\gamma}(z,h)} \leq M_{\ell}$  due to $-M_{\ell} \leq \ell(z, h) \leq \phi_{\gamma}(z, h) \leq \sup _{z \in \gZ} \ell(z, h) \leq M_{\ell}$ and (ii) the Rademacher complexity of the function class $\Phi$ defined by $\mathscr{R}_{i}(\Phi) = \mathbf{E}[\sup _{\phi_{\gamma} \in \Phi} \frac{1}{n_i} \sum_{k=1}^{n_i} \sigma_{k} \phi_\gamma(Z_k,  h_{\theta})] $ where the expectation is w.r.t both $Z_k \stackrel{\text { i.i.d. }}{\sim} P_i$ and i.i.d. Rademacher random variable $\sigma_{k}$ independent of $Z_k, \forall k \in [n_i]$,  we have 
\begin{align}
\sup_{\phi_{\gamma} \in \Phi} \abs*{\mathbf{E}_{Z_i \sim P_i}[\phi_{\gamma}(Z_i, h_{\theta})] -   \mathbf{E}_{Z_i \sim \widehat{P}_{i}}[\phi_{\gamma}(Z_i, h_{\theta})]}  \geq 2 \mathscr{R}_{i}(\Phi)+   M_{\ell} \sqrt{\frac{2 \log (2 m / \delta)}{n_i}} \label{Rade1}
\end{align}
with probability $\leq \delta/m$ due to the standard symmetrization argument and McDiarmid's inequality \blue{[UnderstandingML, Theorem26.5]}. Multiplying $\lambda_i$ to both sides of \eqref{Rade1}, summing up the inequalities over all $i\in [n]$, and using union bound, we obtain \eqref{unionbound1}.


%Conditioning on the vector $Z_1^n \defeq (Z_k)_{k\in [n]}$, the above expectation gives us the empirical Rademacher complexity denoted by $\widehat{\mathscr{R}}_{n}(\Phi)$. 
Define a stochastic process $\left(X_{\phi_{\gamma}}\right)_{\phi_{\gamma} \in \Phi}$ 
$$
X_{\phi_{\gamma}}:=\frac{1}{{\sqrt{n_i}}} \sum_{k=1}^{n_i} \sigma_{k} \phi_{\gamma}(Z_k, h_{\theta})
$$
which is  zero-mean because $\mathbf{E}\left[X_{\phi_{\gamma}}\right]=0$ for all $\phi_{\gamma} \in \Phi$.  To upper-bound  $\mathscr{R}_{n}(\Phi)$, we first show that $\left(X_{\phi_{\gamma}}\right)_{\phi_{\gamma} \in \Phi}$ is a sub-Gaussian process with respect to the following pseudometric
\begin{align}
%\left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{L_2(\widehat{P}_{\lambda})}  \defeq \biggP{\frac{1}{n} \sum_{k=1}^{n}  \BigP{\phi_{\gamma}(Z_k, f_{\theta}) - \phi_{\gamma}(Z_k, h_{\theta'})}^2}^{1/2}. 
\left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{\infty}  \defeq  \sup_{z \in \mathcal{Z}} \Big\lvert  {\phi_{\gamma}(z, h_{\theta}) - \phi_{\gamma}(z, h_{\theta'})}  \Big\rvert . 
\end{align}  

For any $t \in \mathbb{R}$,  using Hoeffding inequality with the fact that $\sigma_{k}, k \in [n]$, are i.i.d. bounded random variable with sub-Gaussian  parameter 1, we have
$$
\begin{aligned}
\mathbf{E}\left[\exp \left(t\left(X_{\phi_{\gamma}}-X_{\phi_{\gamma}^{\prime}}\right)\right)\right] &=\mathbf{E}\left[\exp \left(\frac{t}{\sqrt{n_i}} \sum_{k=1}^{n_i} \sigma_{k}\left(\phi_{\gamma}\left(Z_k, h_{\theta}\right)-\phi\left(Z_k, h_{\theta'}\right)\right)\right)\right] \\
&=\left(\mathbf{E}\left[\exp \left(\frac{t}{{\sqrt{n_i}}} \sigma_{1}\left(\phi_{\gamma}\left(Z_{1}, h_{\theta}\right)-\phi_{\gamma}\left(Z_{1}, h_{\theta'}\right)\right)\right)\right]\right)^{n_i} \\
%& \leq \exp \left(\frac{t^{2} \left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{L_2(\widehat{P}_{\lambda})}^{2}}{2 }\right). 
& \leq \exp \left(\frac{t^{2} \left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{\infty}^2}{2 }\right). 
\end{aligned}
$$
Then, invoking Dudley entropy integral, we have
\begin{align}
\sqrt{n_i}\, {\mathscr{R}}_{i}(\Phi) = \mathbf{E} \sup_{\phi_{\gamma} \in \Phi} X_{\phi_{\gamma}} \leq {12} \int_{0}^{\infty} \sqrt{\log \mathcal{N}\left(\Phi, \norm{\cdot}_{\infty}, \epsilon\right)} \mathrm{d} \epsilon
\end{align}

We will show that when $\theta \mapsto \ell(z,h_{\theta})$ is $L_{\theta}$-Lipschitz, then $\theta \mapsto \phi_{\gamma}(z, h_{\theta})$ is also $L_{\theta}$-Lipschitz. First, we have
\begin{align*}
	\Big|\phi_{\gamma}(z, h_{\theta}) - \phi_{\gamma}(z, h_{\theta'})\Big|  &=  \bigg| \sup_{\zeta \in \mathcal{Z}} \inf_{\zeta' \in \mathcal{Z}} \Big\{ \ell(\zeta,h_{\theta})  - \gamma d(\zeta,  z)   -   \ell(\zeta', h_{\theta'}) + \gamma d(\zeta',  z)  \Big\} \bigg| \\
	&\leq  \bigg| \sup_{\zeta \in \mathcal{Z}} \Big\{ \ell(\zeta,h_{\theta})    -   \ell(\zeta, h_{\theta'})   \Big\} \bigg| \\
	&\leq \sup_{\zeta \in \mathcal{Z}}  \bigg| \Big\{ \ell(\zeta,h_{\theta})    -   \ell(\zeta, h_{\theta'})   \Big\} \bigg| \\
	& \leq L_{\theta}   \norm{\theta - \theta'}, \\
	%& \leq L_f L_{\theta} \norm{\theta - \theta'}
\end{align*}
which implies
\begin{align}
\left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{\infty} \leq  L_{\theta}   \norm{\theta - \theta'}.
\end{align}
Therefore, by contraction principle \blue{[Understanding ML]}, we have
\begin{align}
\mathcal{N}\left(\Phi, \norm{\cdot}_{\infty}, \epsilon\right) \leq \mathcal{N}\left(\Theta, \norm{\cdot}, \epsilon/L_{\theta}\right)
\end{align}
\end{proof}

\begin{proposition}[Measure concentration (Fournier and Guillin, 2015, Theorem 2)]\label{WassRate}
	Let $P$ be a probability distribution on a bounded set $\mathcal{Z}$. Let $\widehat{P}_{n}$ denote the empirical distribution of $Z_{1}, \ldots, Z_{n} \stackrel{\text { i.i.d. }}{\sim} P.$ Assuming that there exist constants $a>1$  such that $A \defeq \mathbf{E}_{Z \sim P}\bigS{\exp(\norm{Z}^a)} < \infty$ (i.e., $P$ is a light-tail distribution). Then, for any $\rho > 0$,
$$
%\mathbf{P}\left[ W (P_{\lambda}, \widehat{P}_{n}) \geq  \rho \right] \leq c_{1} \exp \left(-c_{2} n \rho^{\max\{d+1, 2\}}\right) \\
\mathbf{P}\left[ W (\widehat{P}_{n}, P) \geq  \rho \right]  \leq \begin{cases}c_{1} \exp \left(-c_{2} n \rho^{\max \{d+1,2\}}\right) & \text { if } \rho \leq 1 \\ c_{1} \exp \left(-c_{2} n \rho^{a}\right) & \text { if } \rho>1\end{cases}
$$
where $c_{1}, c_{2}$ are constants depending on $a, A$ and $d$.
\end{proposition}
As a consequence of this proposition,  for any $\delta > 0$, we have  
\begin{align}\label{E:deltarho}
\mathbf{P}\left[ W (\widehat{P}_{n}, P) \leq  \widehat{\rho}_{n}^{\delta} \right] \geq 1 - \delta \; \text{  where  } \; \widehat{\rho}_{n}^{\delta} \defeq \begin{cases}\left(\frac{\log \left(c_{1} / \delta \right)}{c_{2} n}\right)^{\min \{1 / (d+1), 1 / 2\}} & \text { if } n \geq \frac{\log \left(c_{1} / \delta\right)}{c_{2}}, \\ \left(\frac{\log \left(c_{1} / \delta\right)}{c_{2} n}\right)^{1 / \alpha} & \text { if } n<\frac{\log \left(c_{1} / \delta\right)}{c_{2}}.\end{cases}
\end{align}

\begin{corollary}
	With all assumptions as in Theorem~, we have
	\[ 
	\mathscr{L}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}})- \inf_{f \in \mathcal{F}} \mathscr{L}(P_{\lambda}, f) \leq  \sum_{i=1}^{m} \lambda_i \BiggS{\frac{48 \mathscr{C}(\Theta)}{\sqrt{n_i}} + 2 M_{\ell} \sqrt{\frac{2 \log (4  m / \delta)}{n_i}} + \bigP{2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}} }\widehat{\rho}_{n_i}^{\delta/2m} } +\varepsilon
	\]
	with probability at least $1 - \delta$. 
\end{corollary}
\begin{proof}
We will exploit the joint convexity property of 1-Wasserstein distance, which can be shown as the mapping $(\alpha, \beta) \mapsto W(\alpha, \beta)$ is convex. To see that, by Kantorovich-Rubinstein Duality,  we have $W(\alpha, \beta) = \sup_{\norm{f}_L \leq 1} \mathbf{E}_{\alpha}[f] - \mathbf{E}_{\beta}[f] =  \sup_{\norm{f}_L \leq 1} T_f (\alpha, \beta)$, which is the sumpremum of linear functions $T_f: \gP \times \gP \mapsto \mathbb{R}$ defined by $T_f (\alpha, \beta) = (\alpha, \beta)^{\top}(f, -f)$, and thus the convexity follows. Thus we have 
\begin{align}
W(P_{\lambda}, \widehat{P}_{\lambda}) = W \BigP{\sum\limits_{i=1}^m \lambda_i (\widehat{P}_i, P_i)} \leq  {\sum\limits_{i=1}^m \lambda_i W(\widehat{P}_i, P_i)}.
\end{align}
Then, we have
\begin{align}
\mathbf{P}\BigS{W(P_{\lambda}, \widehat{P}_{\lambda}) \geq \sum\limits_{i=1}^{m} \lambda_i \widehat{\rho}_{n_i}^{\delta/2m} }
&\leq \mathbf{P}\BigS{\sum\limits_{i=1}^m \lambda_i W(\widehat{P}_i, P_i) \geq \sum\limits_{i=1}^{m} \lambda_i \widehat{\rho}_{n_i}^{\delta/2m} } \nonumber\\
&\leq \sum\limits_{i=1}^m  \mathbf{P}\BigS{ W(\widehat{P}_i, P_i) \geq   \widehat{\rho}_{n_i}^{\delta/2m} } \nonumber\\
&\leq \sum\limits_{i=1}^m  \frac{\delta}{2 m}= \frac{\delta}{2}, \label{E:barry}
\end{align}
where the second inequality is due to the union bound, and the third inequality is due to  Proposition~\ref{WassRate} and \eqref{E:deltarho}. By setting $\rho = \sum\limits_{i=1}^{m} \lambda_i \widehat{\rho}_{n_i}^{\delta/2m}$  in Theorem~\ref{Thrm:key} and using union bound, we complete the proof. 
\end{proof}

\subsection{How to choose $\lambda$}
Controlling $\lambda$ for various purpose: either adapt to a specific domain or covering all clients with minimum $\rho$. 

For domain adaptation
\begin{align}
\min_{\lambda \in \Delta} W(\widehat{P}_{\lambda}, \widehat{Q}) \leq \min_{\lambda \in \Delta} \sum\limits_{i=1}^{m} \lambda_i W(\widehat{P}_i, \widehat{Q}) 
\end{align}

For covering all client distribution, based on the Wasserstein barycenter problem
\begin{align}
W(\widehat{P}_{{\lambda}^*}, {P}^*) \leq  \min_{\lambda \in \Delta, Q \in \gP} \sum\limits_{i=1}^{m} \lambda_i W(\widehat{P}_i, {Q}) \defeq \rho^*
\end{align}

By triangle inequality:
\begin{align}
W(P_{\lambda^*}, P_j) &\leq W(P_{\lambda^*}, \widehat{P}_{\lambda^*}) + W(\widehat{P}_{\lambda^*}, P^*) + W( P^*, \widehat{P}_j) + W(  \widehat{P}_j, P_j) \nonumber\\
& \leq \sum\limits_{i=1}^{m} \lambda_i^* \widehat{\rho}_{n_i}^{\delta/2m} + \rho^* + \frac{\rho^*}{\lambda_j} + \widehat{\rho}_{n_j}^{\delta/2} \; \text{  with probability at least }  1-\delta, \label{E:bary2}
\end{align}
where \eqref{E:bary2} is due to several facts: (i) $\mathbf{P}\bigS{W(P_{\lambda^*}, \widehat{P}_{\lambda^*}) \geq \sum\limits_{i=1}^{m} \lambda_i^* \widehat{\rho}_{n_i}^{\delta/2m} } \leq \delta/2$ according to \eqref{E:barry}, (ii) $W( P^*, \widehat{P}_j) = \frac{\lambda_j W( P^*, \widehat{P}_j)}{\lambda_j}\leq \frac{\rho^*}{\lambda_j}$, and (iii)  $\mathbf{P}\bigS{W(  \widehat{P}_j, P_j) \geq \widehat{\rho}_{n_j}^{\delta/2} } \leq \delta/2$ according to \eqref{E:deltarho}, and (iv) using union bound. 

\begin{lemma}
\begin{align*}
	\mathscr{L}_{\rho}^{\gamma}(Q, f) & = \mathscr{L}_{\rho}^{\gamma}(Q,f) + \mathscr{L}_{\rho_{\gamma}}^{\gamma}(Q,f) - \mathscr{L}_{\rho}^{\gamma}(Q,f) \\		
	& = \mathscr{L}_{\rho}^{\gamma}(Q, f)+\gamma(\rho - f_{\gamma}) \\
	& \leq  \mathscr{L}(Q, f) + (2L + \gamma\mathbf{I}_{\{\gamma \neq \gamma^{\prime}\}})\rho		
\end{align*}
\end{lemma}

\textbf{Tuning}:
\begin{enumerate}
	\item Choose the desire $\rho^{*}$
	\item Adjust $\gamma$ to have $\rho_{\gamma} = \rho^{*}$
\end{enumerate}



==> sections/related_work.tex <==
\section{Preliminaries}

\subsection{Reinforcement Learning from Human Feedback (RLHF) based on Reward Models}

The RLHF pipeline (Ziegler et al.) usually includes three phases: 

\textbf{a. Supervise Fine-tuning (SFT):} RLHF typically begins by fine-tuning a pre-trained LM with supervised learning (SFT) on high-quality data for the downstream task(s) of interest (dialogue, summarization, etc.), to obtain a model $\pi^{\mathrm{SFT}}$.

\textbf{b. Reward Modeling Phase:}
Next, the SFT model is prompted with prompts $x$ to produce pairs of answers $\left(y_1, y_2\right) \sim \pi^{\mathrm{SFT}}(y \mid x)$. These are then presented to human labelers who express preferences for one answer, denoted as $y_w \succ y_l \mid x$ where $y_w$ and $y_l$ denotes the preferred and dispreferred completion amongst $\left(y_1, y_2\right)$ respectively. \textit{The preferences are assumed to be generated by some latent reward model $r^*(y, x)$, which we do not have access to}.

There are a number of approaches used to model preferences, the \textit{Bradley-Terry (BT) model being a popular choice}. 
%(although more general Plackett-Luce ranking models are also compatible with the framework if we have access to several ranked answers)
The BT model stipulates that the human preference distribution $p^*$ can be written as:
\begin{equation}
    p^*\left(y_1 \succ y_2 \mid x\right)=\frac{\exp \left(r^*\left(x, y_1\right)\right)}{\exp \left(r^*\left(x, y_1\right)\right)+\exp \left(r^*\left(x, y_2\right)\right)} \text{.}
    \label{eq:human_preference}
\end{equation}

Assuming access to a static dataset of comparisons $\mathcal{D}=\left\{x^{(i)}, y_w^{(i)}, y_l^{(i)}\right\}_{i=1}^N$ sampled from $p^*$, we can parametrize a reward model $r_\phi(x, y)$ and estimate the parameters via maximum likelihood. Framing the problem as a binary classification we have the negative log-likelihood loss:
\begin{equation}
\mathcal{L}_R\left(r_\phi, \mathcal{D}\right)=-\mathbb{E}_{\left(x, y_w, y_l\right) \sim \mathcal{D}}\left[\log \sigma\left(r_\phi\left(x, y_w\right)-r_\phi\left(x, y_l\right)\right)\right]
\end{equation}

where $\sigma$ is the logistic function. In the context of LMs, the network $r_\phi(x, y)$ is often initialized from the SFT model $\pi^{\mathrm{SFT}}(y \mid x)$ with the addition of a linear layer on top of the final transformer layer that produces a single scalar prediction for the reward value. To ensure a reward function with lower variance, prior works normalize the rewards, such that $\mathbb{E}_{x, y \sim \mathcal{D}}\left[r_\phi(x, y)\right]=0$ for all $x$.

\textbf{c. RL Fine-Tuning Phase:}
During the RL phase, we use the learned reward function to provide feedback to the language model. In particular, we formulate the following optimization problem
\begin{equation}
    \max _{\pi_\theta} \mathbb{E}_{x \sim \mathcal{D}, y \sim \pi_\theta(y \mid x)}\left[r_\phi(x, y)\right]-\beta \mathbb{D}_{\mathrm{KL}}\left[\pi_\theta(y \mid x) \| \pi_{\mathrm{ref}}(y \mid x)\right]
%5  \label{eq:rl_ft}
\end{equation}

where $\beta$ is a parameter controlling the deviation from the base reference policy $\pi_{\text {ref, }}$, namely the initial SFT model $\pi^{\mathrm{SFT}}$. 

In practice, \textit{the language model policy $\pi_\theta$ is also initialized to $\pi^{\mathrm{SFT}}$}. The added constraint is important, as it prevents the model from deviating too far from the distribution on which the reward model is accurate, as well as maintaining the generation diversity and preventing mode-collapse to single high-reward answers. Due to the discrete nature of language generation, this objective is not differentiable and is typically optimized with reinforcement learning. The standard approach has been to construct the reward function $r(x, y)=r_\phi(x, y)-\beta\left(\log \pi_\theta(y \mid x)-\log \pi_{\mathrm{ref}}(y \mid x)\right)$, and maximize using PPO.

\textbf{Instability of PPO:} Despite its acclaimed effectiveness, recent studies have identified instability associated with PPO. Factors such as reward normalization, reward scaling, reward clipping, KL control, advantage normalization and critic initialization can contribute to this instability. Moreover, we identify another source of instability: there is an inconsistency when it comes to optimizing the reward trained with the Bradley-Terry Loss (BTL) comparative reward model. In essence, BTL is invariant to constant shift while PPO is not. This means that even if two reward models carry identical information about human preferences, optimizing them using PPO can produce different outcomes. 

\subsection{Direct Preference Optimization (DPO)}

Motivated by the challenges of applying reinforcement learning algorithms to large-scale problems such as fine-tuning language models, the goal of DPO is to derive a simple approach for policy optimization using preferences directly. Unlike prior RLHF methods, which learn a reward and then optimize it via RL, DPO leverages a particular choice of reward model parameterization that enables extraction of its optimal policy in closed form, without an RL training loop. As we will describe next in detail, our key insight is to leverage an analytical mapping from reward functions to optimal policies, which enables us to transform a loss function over reward functions into a loss function over policies. This change-of-variables approach avoids fitting an explicit, standalone reward model, while still optimizing under existing models of human preferences, such as the Bradley-Terry model. In essence, the policy network represents both the language model and the (implicit) reward.

\textbf{Deriving the DPO objective}. We start with the same RL objective as prior work, Eq.~\eqref{eq:rl_ft}, under a general reward function $r$. Following prior works, it is straightforward to show that the optimal solution to the KL-constrained reward maximization objective in Eq.~\eqref{eq:rl_ft} takes the form:
\begin{equation}
    \pi_r(y \mid x)=\frac{1}{Z(x)} \pi_{\mathrm{ref}}(y \mid x) \exp \left(\frac{1}{\beta} r(x, y)\right),
    \label{eq:dpo_objective}
\end{equation}
where $Z(x)=\sum_y \pi_{\text {ref }}(y \mid x) \exp \left(\frac{1}{\beta} r(x, y)\right)$ is the partition function. Even if we use the MLE estimate $r_\phi$ of the ground-truth reward function $r^*$, it is still expensive to estimate the partition function $Z(x)$, which makes this representation hard to utilize in practice. However, we can rearrange Eq.~\Cref{eq:dpo_objective} to express the reward function in terms of its corresponding optimal policy $\pi_r$, the reference policy $\pi_{\text {ref }}$, and the unknown partition function $Z(\cdot)$, Specifically, we first take the logarithm of both sides of Eq.~\Cref{eq:dpo_objective} and then with some algebra we obtain:
\begin{equation}
r(x, y)=\beta \log \frac{\pi_r(y \mid x)}{\pi_{\mathrm{ref}}(y \mid x)}+\beta \log Z(x).
\end{equation}

We can apply this reparameterization to the ground-truth reward $r^*$ and corresponding optimal model $\pi^*$. Fortunately, the Bradley-Terry model depends only on the difference of rewards between two completions, i.e., 

\begin{equation}
    p^*\left(y_1 \succ y_2 \mid x\right)=\sigma\left(r^*\left(x, y_1\right)-r^*\left(x, y_2\right)\right).
\end{equation}


Substituting the reparameterization in Eq. 1 for $r^*(x, y)$ into the preference model Eq. \eqref{eq:human_preference}, the partition function cancels, and we can express the human preference probability in terms of only the optimal policy $\pi^*$ and reference policy $\pi_{\text {ref }}$. Thus, the optimal RLHF policy $\pi^*$ under the Bradley-Terry model satisfies the preference model:
\begin{equation}
    p^*\left(y_1 \succ y_2 \mid x\right)=\frac{1}{1+\exp \left(\beta \log \frac{\pi^*\left(y_2 \mid x\right)}{\pi_{\operatorname{ref}}\left(y_2 \mid x\right)}-\beta \log \frac{\pi^*\left(y_1 \mid x\right)}{\pi_{\mathrm{ref}}\left(y_1 \mid x\right)}\right)}
\end{equation}

The derivation is in Appendix A.2. While Eq. 6 uses the Bradley-Terry model, we can similarly derive expressions under the more general Plackett-Luce models [30, 21], shown in Appendix A.3.
Now that we have the probability of human preference data in terms of the optimal policy rather than the reward model, we can formulate a maximum likelihood objective for a parametrized policy $\pi_\theta$. Analogous to the reward modeling approach (i.e. Eq. [2), our policy objective becomes:
\begin{equation}
\mathcal{L}_{\text {DPO }}\left(\pi_\theta ; \pi_{\text {ref }}\right)=-\mathbb{E}_{\left(x, y_w, y_l\right) \sim \mathcal{D}}\left[\log \sigma\left(\beta \log \frac{\pi_\theta\left(y_w \mid x\right)}{\pi_{\text {ref }}\left(y_w \mid x\right)}-\beta \log \frac{\pi_\theta\left(y_l \mid x\right)}{\pi_{\text {ref }}\left(y_l \mid x\right)}\right)\right]
\end{equation}

This way, we fit an implicit reward using an alternative parameterization, whose optimal policy is simply $\pi_\theta$. Moreover, since our procedure is equivalent to fitting a reparametrized Bradley-Terry model, it enjoys certain theoretical properties, such as consistencies under suitable assumption of the preference data distribution [4]. 

%In Section [5, we further discuss theoretical properties of DPO in relation to other works. %What does the DPO update do? For a mechanistic understanding of DPO, it is useful to analyze the gradient of the loss function $\mathcal{L}_{\mathrm{DPO}}$. 
The gradient with respect to the parameters $\theta$ can be written as:

\begin{align}
& \nabla_\theta \mathcal{L}_{\mathrm{DPO}}\left(\pi_\theta ; \pi_{\text {ref }}\right) \nonumber \\
&=  -\beta \mathbb{E}_{\left(x, y_w, y_l\right) \sim \mathcal{D}}\left\Bigg[\underbrace{\sigma\left(\hat{r}_\theta\left(x, y_l\right)-\hat{r}_\theta\left(x, y_w\right)\right)}_{\text {higher weight when reward estimate is wrong }} \right. \label{eq:dpo_gradient} \\ 
& \left. \qquad \qquad \qquad  \qquad \qquad \qquad   \left\Big[\underbrace{\nabla_\theta \log \pi\left(y_w \mid x\right)}_{\text {increase likelihood of } y_w}-\underbrace{\nabla_\theta \log \pi\left(y_l \mid x\right)}_{\text {decrease likelihood of } y_l}\right\Big]\right\Bigg], \nonumber
\end{align}

where $\hat{r}_\theta(x, y)=\beta \log \frac{\pi_\theta(y \mid x)}{\pi_{\mathrm{mf}}(y \mid x)}$ is the reward implicitly defined by the language model $\pi_\theta$ and reference model $\pi_{\mathrm{ref}}$. Intuitively, the gradient of the loss function $\mathcal{L}_{\mathrm{DPO}}$ increases the likelihood of the preferred completions $y_w$ and decreases the likelihood of dispreferred completions $y_l$. Importantly, the examples are weighed by how much higher the implicit reward model $\hat{r}_\theta$ rates the dispreferred completions, scaled by $\beta$, i.e, how incorrectly the implicit reward model orders the completions, accounting for the strength of the KL constraint. Our experiments suggest the importance of this weighting, as a naïve version of this method without the weighting coefficient can cause the language model to degenerate.

\textbf{DPO outline}. The general DPO pipeline is as follows: 1) Sample completions $y_1, y_2 \sim \pi_{\mathrm{ref}}(\cdot \mid x)$ for every prompt $x$, label with human preferences to construct the offline dataset of preferences $\mathcal{D}=\Big\{(x^{(i)}, y_w^{(i)}, y_l^{(i)})\Big\}_{i=1}^N$ and 2) optimize the language model $\pi_\theta$ to minimize $\mathcal{L}_{\mathrm{DPO}}$ for the given $\pi_{\text {ref }}$ and $\mathcal{D}$ and desired $\beta$. In practice, one would like to reuse preference datasets publicly available, rather than generating samples and gathering human preferences. Since the preference datasets are sampled using $\pi^{\mathrm{SFT}}$, we initialize $\pi_{\mathrm{ref}}=\pi^{\mathrm{SFT}}$ whenever available. However, when $\pi^{\mathrm{SFT}}$ is not available, we initialize $\pi_{\text {ref }}$ by maximizing likelihood of preferred completions $\left(x, y_w\right)$, that is, $\pi_{\text {ref }}=\arg \max _\pi \mathbb{E}_{x, y_w \sim \mathcal{D}}\left[\log \pi\left(y_w \mid x\right)\right]$. This procedure helps mitigate the distribution shift between the true reference distribution which is unavailable, and $\pi_{\text {ref }}$ used by DPO.
%Further details related to the implementation and hyperparameters can be found in Appendix $\square$.

\subsection{$\Psi$-PO with identity mapping (IPO)}
IPO defines a new objective called $\Psi$-preference optimization objective ( $\Psi P O$ ):
$$
\max _{\pi_\theta} \underset{\substack{x \sim \rho \\ y_w \sim \pi_\theta(\cdot \mid x) \\ y_l \sim \mu(\cdot \mid x)}}{\mathbb{E}}\left[\Psi\left(p^*\left(y_w \succ y_l \mid x\right)\right)\right]-\tau \mathbb{D}_{\mathrm{KL}}\left[\pi_\theta \| \pi_{\mathrm{ref}}\right],
$$
where $\Psi$ is a general non-decreasing function $\Psi:[0,1] \rightarrow \mathbb{R}$.
Take $\Psi$ to be the identity mapping, IPO derives an off-policy loss on empirical dataset:
$$
\begin{gathered}
\min _{\pi_\theta} \underset{\left\langle x, y_w, y_l, I\right\rangle \sim \mathcal{D}^p}{\mathbb{E}}\left[I h_{\pi_\theta}\left(x, y_w, y_l\right)-(1-I) h_{\pi_\theta}\left(x, y_l, y_w\right) -\frac{\tau^{-1}}{2}\right]^2,
\end{gathered}
$$
where $h_{\pi_\theta}\left(x, y_w, y_l\right)$ is defined as:
$$
h_{\pi_\theta}\left(x, y_w, y_l\right)=\log \frac{\pi_\theta\left(y_w \mid x\right)}{\pi_{\mathrm{ref}}\left(y_w \mid x\right)}-\log \frac{\pi_\theta\left(y_l \mid x\right)}{\pi_{\mathrm{ref}}\left(y_l \mid x\right)} .
$$

IPO claims when preferences are deterministic or near deterministic, DPO will lead over-fitting to the preference dataset at the expense of ignoring the KL-regularation term. And IPO's loss will always regularizes $\pi_\theta$ towards $\pi_{\mathrm{ref}}$ by controlling the gap between the log-likelihood ratios $\log \frac{\pi_\theta\left(y_w \mid x\right)}{\pi_\theta\left(y_l \mid x\right)}$ and $\log \frac{\pi_{\mathrm{ref}}\left(y_w \mid x\right)}{\pi_{\mathrm{ref}}\left(y_l \mid x\right)}$.

Similar to DPO, the IPO loss controls the ratio of $\frac{\pi_\theta\left(y_w \mid x\right)}{\pi_\theta\left(y_l \mid x\right)}$ not too far from $\frac{\pi_{\pi \mathrm{re}}\left(y_w \mid x\right)}{\pi_{\text {rer }}\left(y_l \mid x\right)}$, but doesn't control $\pi_\theta(y \mid x)$ not too far from $\pi_{\mathrm{ref}}(y \mid x)$. When there are not enough constraints, which is almost always the case, the optimal policy is not unique, so the KL-regularation term also fails.


==> sections/related_work_braylon.tex <==
\section{Related Work}

\textbf{RLHF with Explicit/Implicit Reward Model}

The concept of Reinforcement Learning from Human Feedback (RLHF) was initially proposed by \cite{christiano2023deep}. This methodology involves two key phases: firstly, learning a reward model that accurately reflects human preferences, and secondly, employing reinforcement learning algorithms to optimize and maximize these defined rewards. 

The Bradley-Terry Model \cite{bradley1952rank} mentioned in RLHF is a probability model used to assign the “scores" for response to estimate its preference. \cite{dpo} 

\textbf{RLHF with General Preference Model}

\textbf{Self-Play Fine-Tuning}


